A Spatial Modeling Approach for Linguistic Object Data: Analysing dialect sound variations across Great Britain

Dialect variation is of considerable interest in linguistics and other social sciences. However, traditionally it has been studied using proxies (transcriptions) rather than acoustic recordings directly. We introduce novel statistical techniques to analyse geolocalised speech recordings and to explore the spatial variation of pronunciations continuously over the region of interest, as opposed to traditional isoglosses, which provide a discrete partition of the region. Data of this type require an explicit modeling of the variation in the mean and the covariance. Usual Euclidean metrics are not appropriate, and we therefore introduce the concept of $d$-covariance, which allows consistent estimation both in space and at individual locations. We then propose spatial smoothing for these objects which accounts for the possibly non convex geometry of the domain of interest. We apply the proposed method to data from the spoken part of the British National Corpus, deposited at the British Library, London, and we produce maps of the dialect variation over Great Britain. In addition, the methods allow for acoustic reconstruction across the domain of interest, allowing researchers to listen to the statistical analysis.

==> sections/sec-diagnostics.tex <==

\section{Diagnostics and Sound Resynthesis}

  \subsection{Residuals}

  \subsection{Effective number of observations}


==> structure/my-commands.tex <==
\usepackage{pdfsync}
\usepackage{etex} %% to avoid some problems of compatibility?

%% for index
%perhaps change to ``index''
% \usepackage{makeidx}
% \makeindex

%% to have also subsubsections in the TOC
% \setcounter{tocdepth}{4}
% \setcounter{secnumdepth}{5}

\PassOptionsToPackage{dvipsnames}{xcolor}
	\RequirePackage{xcolor} % [dvipsnames]
\definecolor{halfgray}{gray}{0.55} % chapter numbers will be semi transparent .5 .55 .6 .0
\usepackage{tikz}
\usetikzlibrary{calc}

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}



\makeatletter
\setlength{\@fptop}{0pt}  % for aligning all floating figures/tables etc... to the top
\makeatother

\usepackage{graphicx}
\graphicspath{{../figures/}}
\usepackage{grffile}

\usepackage{subfig}
\usepackage{booktabs}
\usepackage{lipsum}
%\usepackage{microtype}
\usepackage{url}
\usepackage[final]{pdfpages}

\usepackage[hyperindex=true]{hyperref}
\hypersetup{pdfborder={0 0 0},
	colorlinks=false,
	linkcolor=black,
	citecolor=black,
        urlcolor=black
}



% to avoid the ``Unicode char \u8: not ...''
\DeclareUnicodeCharacter{00A0}{ }

\usepackage[export]{adjustbox} %% for centering the figures

\usepackage{afterpage} %%

\RequirePackage{float}
\usepackage[maxfloats=25]{morefloats}

\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
% \RequirePackage{amssymb}
% \usepackage{amsfonts}

% \usepackage[refsection=chapter,backend=bibtex]{biblatex}
% \addbibresource{tail/thesis.bib}
\usepackage[authoryear]{natbib}

\usepackage[titletoc,toc,title]{appendix}


% \RequirePackage{booktabs}
\RequirePackage{array}

\usepackage[strict]{changepage}                 % adjust margins for selected portions

\usepackage{enumerate}
\usepackage{xspace}

\usepackage{eqlist}

\usepackage{mathrsfs}

\usepackage[all]{xy}  %% for diagrams!


%% for nomenclature
% \usepackage[refpage]{nomencl}
% \makenomenclature


\usepackage{varioref}
% \RequirePackage[colorlinks,linkcolor=blue, citecolor=blue,urlcolor=blue]{hyperref}

%%%% for notes in the margin
\usepackage{marginnote}
\definecolor{dark-gray}{gray}{0.3}
% \renewcommand*{\marginfont}{\color{gray}\footnotesize\rmfamily}
\renewcommand*{\marginfont}{\color{dark-gray}\footnotesize}

\numberwithin{equation}{section}

% To allow long equations to be breaked
\allowdisplaybreaks[1]

% % % % % % % % % % % % % % % % % Davide % % % % % % % % % % % % % % % %

\usepackage{dsfont}
%\DeclareMathOperator*{\argmin}{arg\,min}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{defn}[thm]{Definition}
\newtheorem{ex}[thm]{Example}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lma}[thm]{Lemma}
\newtheorem{slma}[thm]{Sublemma}
\newtheorem{nota}[thm]{Notation}
\newtheorem{cond}[thm]{Condition}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%% comments & co
\newcommand{\mycom}[1]{ {\color{red} ({\tiny COMMENT} #1)} }
% \newcommand{\scom}[1]{ {\color{red} ({\tiny SHAHIN:} #1)} }

% \usepackage{todonotes}
\newcommand{\todo}[1]{ {\color{red} (#1)} }
% \newcommand{\todo}[1]{}
% \newcommand{\etodo}[1]{ {\color{cyan} (#1)} } % todo eventually
% \newcommand{\etodo}[1]{}
% \newcommand{\ftodo}[1]{ {\color{green} (#1)} } % todo finally, before final submission
% \newcommand{\ftodo}[1]{}
% \newcommand{\details}{{\color{red} (give details)} }
% \newcommand{\details}{}

\newcommand{\supplement}{Appendix\xspace}

%%%%% Specific for BNC paper
\newcommand{\graphdist}{\mathrm{d_g}}  %% the distance on the graph
\newcommand{\england}{\mathcal{E}}
\newcommand{\littleo}{o}
\newcommand{\bigo}{O}
\newcommand{\littleop}{o_\pp}
\newcommand{\bigop}{O_\pp}
\DeclareMathOperator{\symmat}{\mathcal S}
\newcommand{\sing}{\mathrm{sing}}
\newcommand{\latlonspace}{(-90, 90] \times (-180, 180]}
\newcommand{\mfccspace}[1]{\ensuremath{L^2([0,1], \bR^{#1})}}
\newcommand{\spec}[1]{\mathrm{Spec}\left( #1 \right)}
\newcommand{\cep}[1]{\mathrm{Cep}\left( #1 \right)}
\newcommand{\melspec}[1]{\mathrm{MelSpec}\left( #1 \right)}
\newcommand{\mfcc}[1]{\mathrm{MFCC}_{#1}}
%%%%%

% \newcommand{\annot}[1]{\marginpar{\vspace{-1cm}\color{blue}\footnotesize#1}} % annotation
% We remove annotations:
%\newcommand{\annot}[1]{} % annotation

% \newcommand{\bannot}[1]{{\color{green} \footnotesize \texttt{#1} }} % beamer annotation
% \newcommand{\modif}[1]{{\color{cyan}#1}} % for new or modified portion

% Tensor products %% the 'm' or 't' at the end denote the 'm'ultiple-fold or 't'wo-fold tensor product
\DeclareMathOperator*{\tensorm}{\otimes}  % our tensor product
% \newcommand{\tensorm}{\otimes}  % our tensor product
\DeclareMathOperator*{\btensorm}{\bigotimes} % ..and its big version
% \newcommand{\btensorm}{\bigotimes} % ..and its big version
\DeclareMathOperator*{\tensort}{\otimes_2}  % our tensor product
\DeclareMathOperator*{\btensort}{ {\bigotimes}_2} % ..and its big version
% \DeclareMathOperator*{\btensort}{\text{\raisebox{0.25ex}{\scalebox{0.8}{$\bigotimes$}}}_{_2}}
\DeclareMathOperator*{\kprodt}{\: \widetilde{\bigotimes}_2 \:}  % our kronecker product
\DeclareMathOperator*{\kprodm}{\: \widetilde{\bigotimes} \:}  % our kronecker product
% \newcommand{\bkprod}{\widetilde{\bigotimes}}  % ..and its big version
\DeclareMathOperator*{\tkprodt}{\widetilde{\bigotimes}_\tp} % the transpose kronecker product
\DeclareMathOperator*{\atensor}{\odot} %% the algebraic tensor
\DeclareMathOperator*{\tensorpi}{\otimes_{\pi}} %% the algebraic tensor



% Real Hilbert Space
\newcommand{\realH}{H_{\mathbb R}}

% L^{2}(\Omega, H):
\newcommand{\rH}{\mathbb{H}}
% and some subset of \randomH used in the construction of the Cramer representation
\newcommand{\rMo}{{\mathbb{M}_{0}}}
\newcommand{\rM}{{\mathbb{M}}}

% Some ``B''anach spaces
\newcommand{\bspace}{{\mathcal{B}}}
\newcommand{\bprime}{{B'}}

\newcommand{\iid}{i.i.d.\@\xspace}
\newcommand{\simiid}{\stackrel{\mathrm{iid}}{\sim}}

% The margin for a multiline equation
\newlength{\eqmar}
\setlength{\eqmar}{.5cm}

\renewcommand{\sc}[1]{{\left\langle #1 \right\rangle}}
\newcommand{\ssc}[1]{{\langle #1 \rangle}} % smaller version
\newcommand{\HSsc}[1]{\left \langle #1 \right \rangle_{\!\!\mathcal{S}_{2}}}
\newcommand{\HSssc}[1]{\langle #1 \rangle_{\!\mathcal{S}_{2}}} % smaller version

\newcommand{\ud}{{\mathrm{d}}}
\newcommand{\pspace}{{(\Omega, \mathcal{O}, \pp)} }
\newcommand{\brv}{$B$-r.v. }

\newcommand{\e}[1]{\mathfrak{e}_{#1}}

% \newcommand{\ee}{{\mathbb{E} }}
\DeclareMathOperator{\ee}{ \:{\mathbb{E} }}
\newcommand{\eee}[1]{\,\:{\mathbb{E}\left[ #1 \right]}}

\newcommand{\sa}[1]{{\mathcal{ #1 } }}
\newcommand{\saa}{$\sigma$-algebra }
\newcommand{\pp}{{\mathbb{P}}}
\newcommand{\eqd}{{\stackrel{d}{=}}}		% equal in distribution
\newcommand{\convp}{\stackrel{p}{\longrightarrow}}
\newcommand{\convd}{\stackrel{d}{\longrightarrow}}
\newcommand{\convas}{\stackrel{a.s.}{\longrightarrow}}
\newcommand{\rainf}{\rightarrow \infty}
\newcommand{\raz}{\rightarrow 0}
\newcommand{\tp}{{\mathsf{T}}} 	% matrix transpose
\newcommand{\nn}{{\mathcal{N}}}	% normal distr
\newcommand{\rank}[1]{{\mathrm{rank}\left( #1 \right)}}	% rank
\newcommand{\gaus}[2]{\mathcal{N}_{#1}\left( #2 \right)}
% \newcommand{\cgaus}[2]{\mathbb{C}\mathcal{N}_{#1}\left( #2 \right)}
%

\DeclareMathOperator{\cov}{cov}
% \newcommand{\cov}[1]{{\mathrm{cov}}\left( #1 \right)}	% covariance
\newcommand{\var}[1]{{\mathrm{var}}\left( #1 \right)}	% variance
\newcommand{\varX}[1]{{\mathrm{var}_X}\left( #1 \right)}	% variance
\newcommand{\covX}[1]{{\mathrm{cov}_X}\left( #1 \right)}	% covariance
\newcommand{\bias}[1]{{\mathrm{bias}}\left( #1 \right)}	% bias
\newcommand{\trace}[1]{{\mathrm{Tr}\left( #1 \right)}}
%\newcommand{\tracenorm}[1]{{\left\| #1 \right\|_{\mathrm{nuclear}}}}

\newcommand{\vfi}{{\varphi}}
\newcommand{\vep}{{\varepsilon}}

\renewcommand{\ll}{{\mathcal{L}}}

\newcommand{\AIC}{\ensuremath{\text{AIC}}}
\newcommand{\PEN}{\ensuremath{\text{PEN}}}
\newcommand{\GOF}{\ensuremath{\text{GOF}}}


\newcommand{\bT}{\mathbb{T}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mI}{\mathcal{I}}

% Lp spaces
\newcommand{\lL}{{\mathcal{L}^2\left( [0,1] \right) }}
\newcommand{\LL}{{L^2\left( [0,1] \right)}\xspace}
\newcommand{\LLR}{{L^2\left( [0,1], \mathbb{R} \right)}\xspace}
\newcommand{\LLRR}{{L^2\left( [0,1]^{2}, \mathbb{R} \right)}\xspace}
\newcommand{\LLRP}[1]{{L^2\left( [0,1], \mathbb{R}^{#1} \right)}\xspace}
\newcommand{\LLC}{{L^2\left( [0,1], \mathbb{C} \right)}\xspace}
\newcommand{\LLCC}{{L^2\left( [0,1]^{2}, \mathbb{R} \right)}\xspace}
\newcommand{\LLCP}[1]{{L^2\left( [0,1], \mathbb{C}^{#1} \right)}\xspace}
\newcommand{\llp}{{{L^2(\mathbb{P})}}}
\newcommand{\LLOL}{{L^{2}\Big(\Omega, \LLC \Big)}}
\newcommand{\Sob}[1]{\mathcal{W}^{#1}([0,1], \mathbb R)}

\newcommand{\fj}{\mathfrak{j}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fH}{\mathfrak{H}}

\newcommand{\KL}{Karhunen--Lo\`{e}ve\xspace}
\newcommand{\CR}{Cram\'er representation\xspace}
\newcommand{\CKL}{Cram\'er--Karhunen--Lo\`eve\xspace}
\newcommand{\Wlog}{without loss of generality\xspace}
\newcommand{\cadlag}{c\`adl\`ag\xspace}

\newcommand{\lpmy}[1]{$L^{#1}$-$m$-approximability\xspace}
\newcommand{\lpm}[1]{$L^{#1}$-$m$-approximable\xspace}

\newcommand{\limms}[1]{\underset{#1}{\mathrm{l.i.m.}}~}

\newcommand{\indic}[1]{  \mathbf{1}_{ #1 }}
\newcommand{\id}{\mathrm{Id}}
\newcommand{\bt}{{\mathbf{t}}}
\renewcommand{\b}[1]{{\mathbf{#1}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bs}[1]{{\boldsymbol{#1}}}
\newcommand{\bxi}{{\boldsymbol{\xi}}\xspace}
\newcommand{\bvep}{{\boldsymbol{\vep}}}

% \newcommand{\argmax}[1]{{\underset{#1}{\text{argmax}} \:}}
% \newcommand{\argmin}[1]{{\underset{#1}{\text{argmin}} \:}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}


\renewcommand{\vec}[1]{{\text{vec}\left(#1\right)}}

\newcommand{\Imm}{{\mathrm{Im}}}
%\newcommand{\ker}{{\mathrm{Ker}}}
\newcommand{\vspan}{{\mathrm{span}}}

%\DeclareBoldMathCommand\bscriptX{\mathcal{X}}
%\newcommand{\cutx}{{ \bscriptX }}     %for a (random) curve time series X

% \DeclareBoldMathCommand\bbchi{\chi}
% \newcommand{\bchi}{{\bbchi}}     %for a sample curve time series
% \DeclareBoldMathCommand\bbmu{\mu}
% \newcommand{\bmu}{{\bbmu}}     %for the mean of a sample curve time series

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}		%to have small caligraphic letters with \mathpzc

\newcommand{\covK}{\mathpzc{r}}	  %for the cross-covariance Kernel
\newcommand{\covO}{\mathscr{R}}	 %for the cross-covariance Operator

\newcommand{\lsub}[2]{{\vphantom{#2}}_{#1}{#2}}   % produces left subscripts, \lsub{a}{b} is b with left sub a.

\newcommand{\udf}[2]{\widetilde{#1}\,_{#2}}	  % unitary discrete Fourier transform
\newcommand{\zt}[2]{Z_{#1}^{(#2)}}			% The empirical Z at freq #1 of ``order'' #2
\newcommand{\zto}[1]{Z_{\omega}^{(#1)}}			% The empirical Z at freq omega of ``order'' #1
\newcommand{\z}{Z}						% The cramer Z
\newcommand{\specdM}[1]{\Phi_{#1}}		% the spectral density Matrix
\newcommand{\specdK}[1]{\mathpzc{f}_{#1}}	% the spectral density Kernel
% \newcommand{\specdK}[1]{\mathscr{f}_{#1}}	% the spectral density Kernel
\newcommand{\specdKE}[1]{\breve{\mathpzc{f}}_{#1}}	% the spectral density Kernel (asymptotic) Estimator
\newcommand{\specdO}[1]{\mathscr{F}_{#1}}		% the spectral density Operator
\newcommand{\specdOE}[1]{\breve{\mathscr{F}}_{#1}}	% the spectral density Operator (asymptotic) Estimator
\newcommand{\specdB}[1]{\mathbf{f}_{#1}}             % the projection onto the basis of the spectral density
\newcommand{\tspecdB}[1]{\tilde{\b{f}}_{#1}}             % the projection onto the basis of the spectral density
\newcommand{\specdBE}[1]{\breve{\b{f}}_{#1}}             % the projection onto the basis of the asymptotic spectral density

\newcommand{\fdr}{\mathrm{FDR}}
\newcommand{\fdp}{\mathrm{FDP}}

\newcommand{\inLL}{\text{in }L^2}


% \newcommand{\gp}[2]{{\mathcal{N}_{#1}\left( #2 \right)}}

% \DeclareBoldMathCommand\bbfi{\varphi}
% \newcommand{\bfi}{{\bbfi}}     %for orthonormal functions of \Gamma

\newcommand{\ii}{\mathbf{i}\xspace}		% the imaginary number i

\newcommand{\cum}[1]{\mathrm{cum}\left( #1 \right)}	%the cummulant
\newcommand{\cumk}[2]{\mathrm{cum}_{#1}\left( #2 \right)}	%the cummulant
\newcommand{\cumop}[1]{\mathrm{cumop}\left( #1 \right)}	%the cummulant
\newcommand{\scum}{\mathrm{sc}}	%the summed cummulant

%\newcommand{\prok}[1]{\rho \left( #1 \right)}	  % the prokhorov metric
%
%\newtheorem{assump}{Assumption}[subsection]
%\newcommand{\assume}[2]{		% assumption
%
%\vspace*{.5cm}
%\noindent \begin{center} \fbox{  \parbox[c]{.8\columnwidth}{ \begin{assump} \label{#2} #1 \end{assump}  } } \end{center}
%\vspace*{.5cm}
%
%}


%\newcommand{\tset}{{\mathbb{T}}}	   %the time index set
%\newcommand{\rprod}{{\bullet}}		% the scalar product on R^p
%\newcommand{\rnorm}[1]{{\lvert #1 \rvert}}	% the norm on R^p
\newcommand{\rpnorm}[1]{{\left| #1 \right|}}	% the norm on H=L^2
\newcommand{\hnorm}[1]{{\left\lVert #1 \right\rVert}}	% the norm on H=L^2
\newcommand{\hhnorm}[1]{{\lVert #1 \rVert}}	% the norm on H=L^2
%\newcommand{\snorm}[1]{{ {}_{_{\mathpzc{s}}}\!\! \left\lVert #1 \right\rVert}}	% the schatten norm on H=L^2
%\newcommand{\snorm}[1]{ {{  \left\lVert #1 \right\rVert}_{_{\mathpzc{s}}} } }	% the schatten norm on H=L^2
\newcommand{\snorm}[1]{{\left\vert\kern-0.2ex\left\vert\kern-0.2ex\left\vert #1
  \right\vert\kern-0.2ex\right\vert\kern-0.2ex\right\vert}} % its smaller version
\newcommand{\ssnorm}[1]{{\vert\kern-0.2ex\vert\kern-0.2ex\vert #1
  \vert\kern-0.2ex\vert\kern-0.2ex\vert}} % its smaller version
\newcommand{\cnorm}[1]{\left| #1 \right|_{\infty}}
\newcommand{\othernorm}[1]{\lVert #1 \rVert_{*} }
\newcommand{\opnorm}[1]{\snorm{#1}_\infty}
\newcommand{\HSnorm}[1]{\snorm{#1}}
\newcommand{\tnorm}[1]{\snorm{#1}_1}
\newcommand{\ttnorm}[1]{\ssnorm{#1}_1}
\newcommand{\pinorm}[1]{\hnorm{#1}_{\pi}} %% projective norm
% see discussion on http://tex.stackexchange.com/questions/498/mid-vert-lvert-rvert


\newcommand{\te}{\tilde{e}}

\newcommand{\schatten}{\mathcal{S}}
\newcommand{\tc}[1]{\schatten_1(#1)}
\newcommand{\bounded}[1]{\schatten_\infty(#1)}
\newcommand{\HS}[1]{\schatten_2(#1)}

\newcommand{\perm}[2]{\mathrm{Perm}_{#1}\left( #2 \right)}

%% JA Temporary Additions





